CLOAF: CoLlisiOn-Aware Human Flow

Even the best current algorithms for estimating body 3D shape and pose yield results that include body self-intersections. In this paper, we present CLOAF, which exploits the diffeomorphic nature of Ordinary Differential Equations to eliminate such self-intersections while still imposing body shape constraints. We show that, unlike earlier approaches to addressing this issue, ours completely eliminates the self-intersections without compromising the accuracy of the reconstructions. Being differentiable, CLOAF can be used to fine-tune pose and shape estimation baselines to improve their overall performance and eliminate self-intersections in their predictions. Furthermore, we demonstrate how our CLOAF strategy can be applied to practically any motion field induced by the user. CLOAF also makes it possible to edit motion to interact with the environment without worrying about potential collision or loss of body-shape prior.

==> figs/barplot.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t!]
   \begin{center}
   \includegraphics[width=\linewidth]{figs/figs/barplot.pdf}
   \end{center}
   \vspace{-5mm}
   \caption{
      \small{
       \textbf{\bf Self-intersection statistics.} The state-of-the-art HMR 2.0 approach~\cite{Goel23a} recovers bodies with self-intersections in 39.2\% of frames of 3DPW-test set. A recent post-processing method such as~\cite{Pavlakos19a} brings this down to 9.2\%. \Ours{} makes this number all the way to zero.}
}
   \label{fig:barplot}
\end{figure}

==> figs/sota_penetr.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t!]
 \centering
  \includegraphics[width=\linewidth]{figs/sota_penetr_.pdf}
   \caption{
       \small{{\bf Self-intersections in SOTA methods.}.  HMR2.0~\cite{Goel23a} (top row) and PARE~\cite{Kocabas21} (bottom row), two of the best current methods, produce bodies with self-intersections shown in {\it blue}. \Ours{} removes them completely and generates the results shown in {\it gold}.}
}
    \label{fig:sota_penetr}
\end{figure}
